Towards Safe Robot Foundation Models

Robot foundation models hold the potential for deployment across diverse environments, from industrial applications to household tasks. While current research focuses primarily on the policies' generalization capabilities across a variety of tasks, it fails to address safety, a critical requirement for deployment on real-world systems. In this paper, we introduce a safety layer designed to constrain the action space of any generalist policy appropriately. Our approach uses ATACOM, a safe reinforcement learning algorithm that creates a safe action space and, therefore, ensures safe state transitions. By extending ATACOM to generalist policies, our method facilitates their deployment in safety-critical scenarios without requiring any specific safety fine-tuning. We demonstrate the effectiveness of this safety layer in an air hockey environment, where it prevents a puck-hitting agent from colliding with its surroundings, a failure observed in generalist policies.

==> acronyms.tex <==
\RequirePackage{acronym}
\acrodef{octo}[\textsc{octo}]{Octo}
\acrodef{atacom}[\textsc{atacom}]{acting on the tangent space of the constraint manifold}
\acrodef{rfm}[\textsc{rfm}]{Robot foundation model}
\acrodef{vla}[\textsc{vla}]{vision-language-action}
\acrodef{bc}[\textsc{bc}]{behavior cloning}
\acrodef{rl}[\textsc{rl}]{reinforcement learning}
\acrodef{mujoco}[\textsc{mujoco}]{Multi-Joint dynamics with Contact}
\acrodef{cbf}[\textsc{cbf}]{control barrier functions}
\acrodef{hj}[\textsc{hj}]{Hamilton-Jacobi}
\acrodef{vlm}[\textsc{vlm}]{vision-language model}

% Set these variables as already used
\acused{octo}
\acused{rl}
\acused{mujoco}
\acused{atacom}
